Atiyah-Singer Dirac Operator on spacetimes with non-compact Cauchy hypersurface

Let $M$ be a globally hyperbolic manifold with complete spacelike Cauchy hypersurface $\Sigma \subset M$. Building on past and recent works of B\"ar and Strohmaier, we extend their Fredholm result of the Atiyah-Singer Dirac operator on compact Lorentzian spaces to the case, where $M$ is diffeomorphic to a product of $\Sigma$ with a compact time intervall and the hypersurface is a Galois covering with respect to a group $\Gamma$. We follow the first approach of both authors in this extended setting, where a well-posedness result of the Cauchy problem for the Dirac operator on non-compact manifolds is needed in preparation. After employing von Neumann algebras and further ingredients for Galois coverings, the well-posedness result is specified for the setting of interest, which leads to $\Gamma$-Fredholmness of the Dirac operator under APS boundary conditions.

==> footnotes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----------------------------------------------------------------------------- CHAPTER I -----------------------------------------------------------------------------------------------------------%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ---------------------------------------------------------------------------- CHAPTER II -----------------------------------------------------------------------------------------------------------%%


\bnotecontent{f1}{Since each level set is an embedded hypersurface, the inclusion maps $\inclus_t:\, \Sigma_t\,\hookrightarrow\,M$ are smooth embeddings, i.e. $\inclus_t$ are diffeomorphisms between $\Sigma_t$ and $\inclus_t(\Sigma_t)$.}

\bnotecontent{f2}{The term \textit{inward/outward pointing normal vector field} can be rephrased in the Lorentzian setting: if the hypersurface is spacelike, one fixes one of the two timelike normal directions as normal field (here past-directed) and calls it outward pointing. The other time-oriented normal vector is thus the inward pointing normal vector (here future-directed).%This convention is necessary when using Stokes theorem on Lorentzian spaces with spacelike boundary/hypersurfaces.
}
\bnotecontent{f1c}{Here and in the following, if the manifold is clear from the context or from the bundle $E$, we write $C^\infty(E)$ instead of $C^\infty(M,E)$ and the same for other sections.}

\bnotecontent{f3}{We choose the sesquilinearity in such a way, that the first entry is anti-linear.}

\bnotecontent{f4}{Another way of introducing a $\Psi$DO is presented in the appendix \ref{chap:app2} as a Fourier integral operator.}

\bnotecontent{f5}{A more general version of Seeleys result in 1964 can be found in \cite{Melbook} as Theorem and Lemma 1.4.1. in chapter 1.}

\bnotecontent{f11}{In comparison, $L^2_\comp(M,E)$ denotes those sections in $L^2_\loc(M,E)$, having compact support. In order to stress a fixed compact support in $K \Subset M$, I write $$L^2_{K,\loc}(M,E):=\SET{u \in L^2_\loc(M,E)\,\vert\, \supp{u} \subset K}\quad. $$ Then one can define $L^2_\comp(M,E)$ as union of $L^2_{K,\loc}(M,E)$ over all $K$ compact in $M$. }

\bnotecontent{f12}{This follows from the essentially self-adjointness of the identity map and the Bochner Laplacian $\adNabla{E}{}\Nabla{E}{}$, see \cite{BraMilShub} or \cite{yoshida} for detailed proofs. It holds true for any compact manifold, since they are complete by the Hopf-Rinow theorem.}

\bnotecontent{f13}{If one has $k+\alpha < s-\frac{\dim(M)}{2}$ with $\alpha \in \intervallo{}{0}{1}$, one has even more a continuous embedding into the Hölder spaces $C^{k,\alpha}(M,E)$.}

\bnotecontent{f27}{In comparison the \textit{domain of dependence} (also known as \textit{"causal diamond"}) is defined as $\domdep{}(A)=\domdep{+}(A)\cup \domdep{-}(A)$ for $A \subset M$, such that no two contained points can be connected by a timelike curve (i.e. $A$ is achronal), where
\begin{equation*}
\domdep{\pm}(A):=\SET{p \in M\,\vert\,\text{every past}(+)\setminus\,\text{future}(-)\,\text{inextendible causal curve through}\,p\,\text{meets}\,A}\quad.
\end{equation*}
In particular $A \subset \domdep{\pm}(A)$, but also $\domdep{\pm}(A)\subset\Jlight{\pm}(A)$. }

\bnotecontent{fc1}{Later on $\mathcal{M}=\Sigma$ or $\Sigma_t$ for a $t \in \timef(M)$.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----------------------------------------------------------------------------- CHAPTER III ---------------------------------------------------------------------------------------------------------%%

\bnotecontent{f6}{Thus it is an oriented manifold together with a $\group{Spin}_0(1,n)$-principal bundle, where 
\begin{equation*}
\group{Spin}_0(1,n):=\SET{e_1,...,e_{2k}\in \group{Cl}^0_{1,n}\,\vert\,v_j \in \R^{n+1}\, , \, \idscal{1}{}{v_j}{v_j}=\pm 1 \quad \text{and} \quad \prod_{j=0}^{2k}\idscal{1}{}{v_j}{v_j}=1}
\end{equation*}
with $\group{Cl}^0_{1,n}$ as even elements of the Clifford-algebra w.r.t. the symmetric bilinearform $\idscal{1}{}{\cdot}{\cdot}$ is the connected component of the identity in the spin group; see \cite{BaerGauMor} and related literature for more details.}

\bnotecontent{f10}{Sections of $\spinb^{\pm}(\Sigma_t)$ for each hypersurface can be interpreted as spinor fields on the hypersurface with positive or negative chirality, even though I used it as $\spinb^{\pm}(\Sigma_{t})=\spinb^{\pm}(M)\vert_{\Sigma_t}=\spinb(\Sigma_t)$ for both signs. But since I won't apply a chirality decomposition on the hypersurfaces, this shouldn't bother here.}

\bnotecontent{f14}{See Proposition 1.3.5 in \cite{Gin} or the orginal proof of Theorem 1.17. in \cite{GroLaw}.}

\bnotecontent{f28}{Manifolds with bounded geometry are complete, which follows from the injectitivity radius condition; see Definition 1.1 in \cite{shubinspec} and following. Thus, the results from the former sections can be applied.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----------------------------------------------------------------------------- CHAPTER IV ----------------------------------------------------------------------------------------------------------%%

\bnotecontent{f7}{This circumstand might lead to an obstruction in using more general boundary conditions as e.g. given in \cite{BaerHan} paragraph 4.2., where the multiplicities induce an additional term in the index formula for the compact case, if one is using this kind of generalized Atiyah-Patodi-Singer boundary conditions.}

\bnotecontent{f8}{The same procedure will be applied for the flip metric of $\met$ in order to compute the geometric index formula.}

\bnotecontent{f9}{It is also possible to achieve, that every leave $\mathcal{T}=const$ in a globally hyperbolic manifold is complete and a Cauchy hypersurface by modifying the lapse function $N$ to be bounded on every leave; this shown in Proposition 15 in \cite{mueller}.}

\bnotecontent{f15}{See appendix \ref{chap:app2} for the notations.}

\bnotecontent{f20}{This as well can be seen in Definition \ref{defevop}, since the Dirac wave evolution operator maps compactly supported Sobolev-sections to compactly supported Sobolev-sections and is a topological isomorphism, so its adjoint does as well.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----------------------------------------------------------------------------- CHAPTER V ----------------------------------------------------------------------------------------------------------%%

\bnotecontent{f16}{The boundness on $\kernel{B}$ is inherited from the boundness on $\mathscr{H}$.}

\bnotecontent{f17}{Equivalently, the orbit of each point in $M$ is $M$ itself.}

\bnotecontent{f18}{Another reference for the Dirac operator on a Riemannian $\Upgamma$-manifold is Proposition 3.1 in \cite{atiyahellvn}.}

\bnotecontent{f19}{$B\ydo{\ast}{(\mathsf{cl})}$ is closed under composition.}

\bnotecontent{f29}{Shubin introduced in \cite{shub} this class to consist of those pseudo-differential operators, which differ from a properly supported pseudo-differential operator by just a smoothing operator in $\ydo{-\infty}{\Upgamma}$. But the definition given here coincides with the manner, how these operators have been actually used in this reference.}

\bnotecontent{f21}{See e.g. Theorem 3.2. \cite{Joshi} for the more general statement, that the tensor product of two local Sobolev sections is again a local section.}

\bnotecontent{f22}{Since $\upnu$ is chosen to be globally past-directed, the temporal projection of $\zeta_{+}$ is anti-parallel to $\upnu$, whereas the projection of $\zeta_{-}$ in temporal direction is parallel; the same holds for $\varsigma_{\pm}$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----------------------------------------------------------------------------- CHAPTER VI ---------------------------------------------------------------------------------------------------------%%

\bnotecontent{f23}{Projections on a Banach space are bounded iff their kernels and range are closed subspaces of this Banach space.}

\bnotecontent{f24}{See \cite{benroy} Appendix A for the identification an operator $A \in \mathscr{K}_\Upgamma(\mathscr{H}_1,\mathscr{H}_2)$ to correspond to an operator $\tilde{A}$, mapping as compact operator between the Hilbert spaces $\mathcal{H}_1$ and $\mathcal{H}_2$, i.e. $(\id{}\otimes\tilde{A}) \in \mathcal{N}_{r}(\Upgamma)\otimes\mathscr{K}(\mathcal{H}_1,\mathcal{H}_2)$.}

\bnotecontent{f25}{Here and in the following of this proof every appearing topological isomorphism between Hilbert $\Upgamma$-modules can be considered as unitary isomorphism; see Proposition in section 2.16. of \cite{shub}. Thus every appearing isomorphism between Hilbert $\Upgamma$-modules implies, that their $\Upgamma$-dimensions coincide.}

\bnotecontent{f26}{The mixed terms can be estimated with the polarization identity of the form
\begin{equation*}
4\Rep{\dscal{1}{\mathcal{H}}{x}{y}}=\norm{x+y}{\mathcal{H}}^2-\norm{x-y}{\mathcal{H}}^2 \leq \norm{x+y}{\mathcal{H}}^2+\norm{x-y}{\mathcal{H}}^2 = 2\norm{x}{\mathcal{H}}^2+2\norm{y}{\mathcal{H}}^2
\end{equation*}
for $x,y\in \mathcal{H}$ Hilbert space. This explains the factor 2 in the third line, which will be restored into the constant in front.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%----------------------------------------------------------------------------- APPENDIX -------------------------------------------------------------------------------------------------------------%%

\bnotecontent{af1}{See \cite{nazaetal} and \cite{sipa} for more details.}

\bnotecontent{af2}{Certain wavefront set conditions have to hold for both cases in addition and for each case a transversality condition: Let 
\begin{equation*}
N^\ast\mathrm{graph}(f):=\SET{(x,\xi,y,\eta)\in T^\ast(X\times Y)\,\vert\, y=f(x) \quad\text{and}\quad \xi\in(\differ f\vert_x)^{\dagger}(\SET{\eta})}\subset T^\ast X \times T^\ast Y
\end{equation*}
denote the conormal bundle of the graph of $f$, then $\mathsf{s}^\ast(N^\ast\mathrm{graph}(f))\pitchfork T^\ast X \times \mathsf{\Lambda}_Y$ for the pullback and \\
$\mathsf{s}^\ast(N^\ast\mathrm{graph}(f))\pitchfork \mathsf{\Lambda}_X \times T^\ast Y$ for the pushforward. $\mathsf{\Lambda}_X$ and $\mathsf{\Lambda}_Y$ are Lagrangian submanifolds of the mapped Lagrangian distributions and $(\differ f\vert_p)^{\dagger}\,:\,T^\ast_{f(p)}Y\,\rightarrow\,T^\ast_p X$ is the adjoint map of the pushforward, which is a priori defined for $f$ being a diffeomorphism, but used here for the preimage.}

